Graphs with large minimum degree and no small odd cycles are $3$-colourable

Answering a question by Letzter and Snyder, we prove that for large enough $k$ any $n$-vertex graph $G$ with minimum degree at least $\frac{1}{2k-1}n$ and without odd cycles of length less than $2k+1$ is $3$-colourable. In fact, we prove a stronger result that works with a slightly smaller minimum degree.

==> Tikz/CaseA.tex <==
\begin{tikzpicture}[scale=1.3]
\draw[] ($(1.3,0)+(-180:1.3)$) arc (-180:180:1.3cm);
\draw[] ($(-3.9,0)+(-180:1.3)$) arc (-180:180:1.3cm);
\node[] () at ($(-2.7,1.3)$) {\small{$C_1$}};
\node[] () at ($(0,1.3)$) {\small{$C_2$}};


\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0cm]180:\scriptsize{$p_1$}}] (Vu) at ($(-1.3,0)+(-180:1.3)$) {};
\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0cm]0:\scriptsize{$p_2$}}] (t) at ($(0,0)$) {};
\draw[] (Vu) -- (t);
\node[label={[label distance=-0.08cm]90:\scriptsize{$P$}}] () at ($(-1.3,0)$) {};




\begin{scope}[on background layer]
\draw[line width=10pt, color=blue!20, line cap=round] ($(1.3,0)+(50:1.3)$) arc (50:310:1.3cm);
\node[] () at ($(0,-1.3)$) {\textcolor{blue}{\small{$B_2$}}};

\draw[line width=10pt, color=blue!20, line cap=round] ($(-3.9,0)+(-165:1.3)$) arc (-165:165:1.3cm);
\node[] () at ($(-2.6,-1.3)$) {\textcolor{blue}{\small{$B_1$}}};
\end{scope}









\end{tikzpicture}

==> Tikz/CaseB.tex <==
\begin{tikzpicture}[scale=1.3]
\draw[] ($(1,0)+(-180:1.3)$) arc (-180:180:1.3cm);
\draw[] ($(-2,0)+(-180:1.3)$) arc (-180:180:1.3cm);
\node[] () at ($(-2,1)$) {\small{$C_1$}};
\node[] () at ($(1,1)$) {\small{$C_2$}};


%\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0cm]180:\scriptsize{$p_1$}}] (Vu) at ($(-1.3,0)+(-180:1.3)$) {};

\foreach \x/\y/\z in {x_2/30/210, s_1'/-40/140, s_1/-90/90, x_1/-120/60}{
\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0.1cm]\z:\scriptsize{$\x$}}] (\x) at ($(-2,0)+(\y:1.3)$) {};
}

\foreach \x/\y/\z in {s_2'/-140/40, s_2/-90/90}{
\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0.1cm]\z:\scriptsize{$\x$}}] (\x) at ($(1,0)+(\y:1.3)$) {};
}

\draw (-0.5,-2.7) ellipse (3.4cm and 1cm);
\node[] () at ($(-0.5,-2)$) {\small{$C_3$}};


\begin{scope}[on background layer]
\draw[line width=10pt, color=blue!20, line cap=round] ($(-2,0)+(45:1.3)$) arc (45:375:1.3cm);
\node[] () at ($(-2.9,0)$) {\textcolor{blue}{\small{$P_1$}}};

\draw[line width=10pt, color=blue!20, line cap=round] ($(1,0)+(-175:1.3)$) arc (-175:80:1.3cm);
\node[] () at ($(1.8,0)$) {\textcolor{blue}{\small{$P_2$}}};
\draw[] (s_1')--(s_2');
\node[] () at ($(-0.5,-1.1)$) {\small{$P'$}};

\draw[line width=10pt, color=gray!50, line cap=round] (x_2) -- ($(x_2)+(0.7,0)$);

\draw[line width=10pt, color=gray!50, line cap=round] (s_1) -- ($(s_1)+(0,-0.5)$);
\draw[line width=10pt, color=gray!50, line cap=round] (s_2) -- ($(s_2)+(0,-0.5)$);
\end{scope}









\end{tikzpicture}

==> Tikz/CaseC.tex <==
\begin{tikzpicture}[scale=1.3]
\draw[] ($(1,0)+(-180:1.3)$) arc (-180:180:1.3cm);
\draw[] ($(-2,0)+(-180:1.3)$) arc (-180:180:1.3cm);
\draw[] (-0.5,-2.7) ellipse (3.4cm and 1cm);
\node[] () at ($(-2,1)$) {\small{$C_1$}};
\node[] () at ($(1,1)$) {\small{$C_2$}};


%\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0cm]180:\scriptsize{$p_1$}}] (Vu) at ($(-1.3,0)+(-180:1.3)$) {};

\foreach \x/\y/\z in {x_2/30/210, s_1/-90/90, x_1/-120/60}{
\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0.1cm]\z:\scriptsize{$\x$}}] (\x) at ($(-2,0)+(\y:1.3)$) {};
}

\foreach \x/\y/\z in {s_2/-90/90}{
\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0.1cm]\z:\scriptsize{$\x$}}] (\x) at ($(1,0)+(\y:1.3)$) {};
}

\node[circle, draw, inner sep=0pt, minimum width=4pt, color=black, fill=black!20, label={[label distance=-0.1cm]270:\scriptsize{$s_3$}}] () at ($(s_2)+(0,-0.5)$) {};


\node[] () at ($(-0.7,-1.3)$) {\small{$P''$}};
\node[] () at ($(-0.5,-2)$) {\small{$C_3$}};

\draw ($(-0.5, -2.7) + (95:3.4cm and 1cm)$) -- ($(-2,0)+(-50:1.3)$);

\begin{scope}[on background layer]
\draw[line width=10pt, color=blue!20, line cap=round] ($(-2,0)+(45:1.3)$) arc (45:375:1.3cm);

\draw[line width=10pt, color=blue!20, line cap=round] ($(-0.5, -2.7) + (-150:3.4cm and 1cm)$(P) arc (-150:100:3.4cm and 1cm);

\node[] () at ($(-2.9,0)$) {\textcolor{blue}{\small{$P_1$}}};
\node[] () at ($(2.5,-2.7)$) {\textcolor{blue}{\small{$P_3$}}};
\draw[line width=10pt, color=gray!50, line cap=round] (x_2) -- ($(x_2)+(0.7,0)$);

\draw[line width=10pt, color=gray!50, line cap=round] (s_1) -- ($(s_1)+(0,-0.5)$);
\draw[line width=10pt, color=gray!50, line cap=round] (s_2) -- ($(s_2)+(0,-0.5)$);
\end{scope}









\end{tikzpicture}
